Predicting SMT Solver Performance for Software Verification

The Why3 IDE and verification system facilitates the use of a wide range of Satisfiability Modulo Theories (SMT) solvers through a driver-based architecture. We present Where4: a portfolio-based approach to discharge Why3 proof obligations. We use data analysis and machine learning techniques on static metrics derived from program source code. Our approach benefits software engineers by providing a single utility to delegate proof obligations to the solvers most likely to return a useful result. It does this in a time-efficient way using existing Why3 and solver installations - without requiring low-level knowledge about SMT solver operation from the user.

==> eptcsdata.tex <==
\providecommand{\firstpage}{20}
\providecommand{\publicationstatus}{C. Dubois, P. Masci, D. M\'ery (Eds.): F-IDE 2016\\
EPTCS 240, 2017, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.240.2}{10.4204/EPTCS.240.2}}
\pdfoutput=1

